General Evaluation for Instruction Conditioned Navigation using Dynamic Time Warping

In instruction conditioned navigation, agents interpret natural language and their surroundings to navigate through an environment. Datasets for studying this task typically contain pairs of these instructions and reference trajectories. Yet, most evaluation metrics used thus far fail to properly account for the latter, relying instead on insufficient similarity comparisons. We address fundamental flaws in previously used metrics and show how Dynamic Time Warping (DTW), a long known method of measuring similarity between two time series, can be used for evaluation of navigation agents. For such, we define the normalized Dynamic Time Warping (nDTW) metric, that softly penalizes deviations from the reference path, is naturally sensitive to the order of the nodes composing each path, is suited for both continuous and graph-based evaluations, and can be efficiently calculated. Further, we define SDTW, which constrains nDTW to only successful paths. We collect human similarity judgments for simulated paths and find nDTW correlates better with human rankings than all other metrics. We also demonstrate that using nDTW as a reward signal for Reinforcement Learning navigation agents improves their performance on both the Room-to-Room (R2R) and Room-for-Room (R4R) datasets. The R4R results in particular highlight the superiority of SDTW over previous success-constrained metrics.

==> discussion.tex <==

\section{Evaluation}
\label{sec:discussion}

To assess the utility of nDTW as a measure of similarity between two paths, we compare its correlation with human judgments for simulated paths in the context of other standard metrics. Further, we demonstrate that it is advantageous to use it as a reward signal for RL agents on the Room-to-Room (R2R) task \cite{anderson2018vision} and its Room-for-Room (R4R) extension \cite{jain2019stay}.

\subsection{Human evaluations}

To better understand how evaluation metrics behave, we turn to human judgment. As illustrated in Figure \ref{img:human_evals}, we give human raters a series of questionnaires each containing a set of five reference (shown in blue) and query (shown in orange) path pairs. In each set, we keep the reference path fixed and instruct raters to ask themselves the following question when ranking the path pairs: \textit{``If I instructed a robot to take the blue path, which of these orange paths would I prefer it to take?"}

The environment and paths are randomly generated. The environment consists of $15{\times}15$ nodes, forming an approximate grid. Each node $n_{ij}$, $1 \le i, j \le 15$ has coordinates $(x_{ij}, y_{ij})$, where $x_{ij} \sim U(i-\zeta, i+\zeta)$ and $y_{ij} \sim U(j-\zeta, j+\zeta)$ are independently drawn according to a parameter $\zeta$ set to $0.3$. For every pair of nodes $n_{i_1j_1}$ and $n_{i_2j_2}$, we take the Euclidean distance between their coordinates $\lVert n_{i_1j_1}  n_{i_2j_2} \rVert$ and connect them with an edge if and only if $\lVert n_{i_1j_1}  n_{i_2j_2} \rVert \le 1.4$. Each path is generated according to a random procedure: first, a random node is drawn; then, a node two or three edges away is chosen, and this step is repeated. The final path is the shortest path connecting adjacent nodes from this procedure. Figure \ref{img:human_evals} illustrates some of these paths. As in \citet{anderson2018vision}, we set the success threshold to be $1.33$ times the average edge length in the environment.

\begin{figure*}
\centering
\includegraphics[width=.9\linewidth]{img/human_evals.png}
\caption{Example comparison set with one reference path (blue) and five query paths (orange) for human raters to rank according to their preferences.}
\label{img:human_evals}
\end{figure*}

\gamaga{Suggestion: remove this table and include numbers similar to what Jason computed and we included in the rebuttals. Do we have the full numbers?}


\begin{table}
\setlength\tabcolsep{4pt}
    \centering
    \begin{tabu}{lcccccccccccc}
    Scenario & PL & NE & ONE  & SR & OSR & AD & MD & SPL & SED & CLS & nDTW & SDTW\\\hline
    \multirow{2}{*}{UC} & .15 & .70 & .60  & .25 & .30 & .75 & .69 & .26 & .30 & .57 & \textbf{.76} & .25\\ 
    \rowfont{\scriptsize}
       & $\pm$ .53 & $\pm$ .37 & $\pm$ .43 & $\pm$ .53 & $\pm$ .51 & $\pm$ .33 & $\pm$ .33 & $\pm$ .51 & $\pm$ .49 & $\pm$ .49 & \textbf{$\pm$ .33} & $\pm$ .54\\\noalign{\vskip .05in}  
    \multirow{2}{*}{SC} & .01 & .20 & .15  & n/a & n/a & .74 & .68 & .12 & .16 & .73 & \textbf{.81} & \textbf{.81}\\
    \rowfont{\scriptsize}
       & $\pm$ .53 & $\pm$ .54 & $\pm$ .55 & n/a & n/a & $\pm$ .31 & $\pm$ .37 & $\pm$ .53 & $\pm$ .54 & $\pm$ .31 & \textbf{$\pm$ .28} &\textbf{ $\pm$ .28} \\\noalign{\vskip .05in}  
    \end{tabu}
    \caption{Average and standard deviation of Spearman's rank correlations of navigation metrics and human rankings, on unconstrained (UC) and success-constrained (SC) scenarios. See Table \ref{tab:nav-metrics} for definition of each metric.}
    \label{tab:human_evals}
\end{table}

Since some metrics only give a score greater than zero if the success criteria is met, we study two scenarios, \textit{unconstrained} (UC) and \textit{success-constrained} (SC). In the first, query paths are randomly generated without constrains, while in the second, exemplified in Figure \ref{img:human_evals}, only query paths that meet the success criteria are considered.

We collect annotations on 2525 samples (505 sets of 5 query and reference pairs) from 9 human raters, split between UC (1325 samples) and SC (1200 samples). Each set is ranked according to the metrics in Table \ref{tab:nav-metrics}. Once scores are computed, we compare the rankings of each metric with the ones generated by humans, and calculate the average Spearman's rank correlation \cite{spearman1904proof}. The correlation scores are shown in Table \ref{tab:human_evals}, for all metrics metrics presented in Table \ref{tab:nav-metrics}.

The AD and MD numbers show that such simple measures are often better than more complex ones. Nonetheless, nDTW still beats both of them handily across both UC and SC. Furthermore, the lower standard deviation for nDTW compared to all others shows that it more consistently agrees with human rankings across all samples. 



\subsection{Evaluation on VLN Tasks}

We demonstrate a practical application of nDTW, by using it as a reward signal for agents in the Matterport3D environment \cite{Matterport3D}, on both the R2R \cite{anderson2018vision} and R4R datasets \cite{jain2019stay}. Unlike R2R, which contains only direct-to-goal reference paths, R4R contains more convoluted paths that might even come back to their starting point. In the latter scenario, the overly simplistic nature of metrics that use only the last node in the reference path to evaluate performance becomes more evident.

We follow the experimental settings of \citet{jain2019stay}, and train agents using our own implementation. As a baseline, we follow \citet{jain2019stay} for evaluating random agents, by sampling the number of steps from the distribution of those of reference paths in the datasets. Each step is taken by uniformly sampling between possible neighbors. We report the metrics by averaging them across 1 million of these random trajectories.



Our \textit{goal-oriented} agent receives at each transition $q_i \rightarrow q_{i+1}$ a reward equal to to how much closer it got to its final goal---$d(q_{i}, r_{|R|}) - d(q_{i+1}, r_{|R|})$. At the end of each episode, the agent receives a completion reward of +1 if it succeeded ($d(q_{|Q|}, r_{|R|}) \le d_{th}$, where $d_{th} = 3$m for the Matterport3D environment) and -1 otherwise. Although this is equivalent of the \textit{goal-oriented} reward of \citet{jain2019stay}, we obtained performance numbers generally higher than those in their work, due to differences in hyper-parameters and implementation details. Our \textit{fidelity-oriented} agent uses nDTW, receiving at each transition a reward proportional to the gain $\textrm{nDTW}(q_{1..i+1}, R) - \textrm{nDTW}(q_{1..i}, R)$. At the end of each episode, the agent receives a non-zero reward only if the success criteria is met, equal to a linear function of its navigation error: $1 - d(q_{|Q|}, r_{|R|}) / d_{th}$.

%+1 if the agents ends precisely on its goal and of 0 if the distance to the goal is equal to $d_{th} = 3$m.

The metrics on the random, goal-oriented and fidelity-oriented agents are shown in Table \ref{tab:rxr}. Compared to a goal-oriented reward strategy, taking advantage of nDTW as a reward signal leads to comparable or better performance as measured by previous metrics, and strictly better performance as measured by both nDTW and SDTW. nDTW shows better differentiation compared to CLS on R4R between goal and fidelity oriented agents. SED scores random paths more highly than those of trained agents, and neither SR nor SED differentiate between goal and fidelity orientation. SPL appears to do so (15.0 vs 21.4), but this is only due to the fact that the fidelity-oriented agent produces paths that have more similar length to the reference paths rather than fidelity to them. As such, SDTW provides the clearest signal for indicating both success and fidelity.


\begin{table*}
\centering
% \def\arraystretch{0.95}
\setlength\tabcolsep{2.9pt}
\begin{tabular}{lcccccccccccc}
  & \multicolumn{6}{c}{\textbf{R2R}} & \multicolumn{6}{c}{\textbf{R4R}}\\\cmidrule(lr{0.2cm}){2-7}\cmidrule{8-13}
Agent                            & SR & SPL & SED & CLS & \underline{nDTW} & \underline{SDTW} &  SR & SPL & SED & CLS & \underline{nDTW} & \underline{SDTW}\\\hline\noalign{\vskip .02in}
random & 5.1 & 3.3 & 5.8 & 29.0 & 27.9 & 3.6 & 13.7 & 2.2 & 16.5 & 22.3 & 18.5 & 4.1 \\
goal-oriented & 43.7 & 38.4 & 31.9 & 53.5 & 54.4 & 36.1 & \textbf{28.7} & 15.0 & \textbf{9.6} & 33.4 & 26.9 & 11.4 \\
fidelity-oriented & \textbf{44.4} & \textbf{41.4} & \textbf{33.9} & \textbf{57.5} & \textbf{58.3} & \textbf{38.3} & 28.5 & \textbf{21.4} & 9.4 & \textbf{35.4} & \textbf{30.4} & \textbf{12.6} \\
\end{tabular}
\caption{Evaluation metrics as percentages on R2R and R4R Validation Unseen sets for agents with different reward functions. In all metrics, higher means better.\label{tab:rxr}}
\end{table*}


==> dtw.tex <==
\section{Dynamic Time Warping}
\label{sec:dtw}

DTW is computed by aligning elements from a reference and a query series, preserving the order in which elements appear in each of them, and forcing the initial and final elements of the query series to be aligned those of the reference series. Formally, let $R = r_{1..|R|}$ and $Q = q_{1..|Q|}$ be the reference and query series, where $r_i \in \mathcal{F}, 1 \le i \le |R|$ and $q_j \in \mathcal{F}, 1\le j \le |Q|$ for some feature space $\mathcal{F}$ (in the context of navigation, for instance, $\mathcal{F}$ is the space of navigable points in space). Let $\delta: \mathcal{F}\times \mathcal{F} \rightarrow \mathbb{R}_{\ge 0}$ be a distance function mapping pairs of elements in the feature space $\mathcal{F}$ to a real non-negative number. Let $W = w_{1..|W|}$ be a \textit{warping} where $w_k = (i_k, j_k) \in [1:|R|] \times [1:|Q|]$ for $1 \le k \le |W|$, satisfying the two conditions below:

\begin{itemize}
    \item[(i)] \textit{Boundaries:} $w_1 = (1,1)$ and $w_{|W|} = (|R|, |Q|)$;
    \item[(ii)] \textit{Step size:} $w_{k+1} - w_k \in {(1, 1), (1, 0), (0, 1)}$, for every $1\le k < |W|$.
\end{itemize}

From (ii), a \textit{monotonicity} property can also be derived: it follows that $i_{k} \le i_{k+1}$ and $j_{k} \le j_{k+1}$, for every $1\le k < |W|$, ensuring the the warping preservers ordering. Finally, let $\mathcal{W}$ be the set of all valid warpings. Intuitively, $\mathcal{W}$ defines a space of non-linear, order-preserving warpings between the two sequences, respecting the alignment between the initial and final elements in them.



DTW then finds the optimal ordered alignment between the two series by minimizing the cumulative cost of the warping. Formally:

\begin{equation}
    \text{DTW}(R, Q) = \min_{W \in \mathcal{W}} \sum_{(i_k, j_k) \in W} \delta(r_{i_k}, q_{j_k}).
\end{equation}



% In the pseudo-code, the variable \textit{search\_cells} is an array that stores, in an ordered fashion, all cells ($i$ and $j$ coordinates) to be searched: for every indices $k_1$ and $k_2$ where $k_2 > k_1$, let $(i_1, j_1) = \textrm{search\_cells}[k_1]$ and $(i_2, j_2) = \textrm{search\_cells}[k_2]$, then it is true that $(i_2 > i_1) \lor ((i_2 = i_1) \wedge (j_2 > j_1))$. Given a position $k$ associated with the cell $(i, j)$, it is then possible to find the positions of the cells $(i-1, j)$, $(i, j-1)$ and $(i-1, j-1)$ in constant time, since their difference is limited by the search radius. In the pseudo-code, this is done by the procedure \textit{try\_find}, that receives a position $(i, j)$ to look for, a heuristic $k$ and the list of \textit{search\_cells}, returning -1 if it is not found. The method \textit{get} is then used to try to get the value of an array at a given position, returning a default value in case the position is invalid.


% \begin{algorithm}
% \caption{FastDTW (linear space and time complexities)}
% \begin{algorithmic} 
% \Procedure{FastDTW}{$R$, $Q$, search\_radius}
% \State min\_resolution$\leftarrow$search\_radius + 2
% \If{$|R| \le $ min\_resolution or $|Q| \le $ min\_resolution}

% \Return DTW(R, Q)\Comment{Fall back to quadratic complexity DTW computation.}
% \Else

% \LineComment{Reduce resolution for both series.}
% \State shrunk\_$R$ $\leftarrow$ reduce\_by\_half($R$)
% \State shrunk\_$Q$ $\leftarrow$ reduce\_by\_half($Q$)
% \State

% \LineComment{Recursively get lower-resolution warping.}
% \State low\_res\_dtw, low\_res\_path $\leftarrow$ FastDTW(shrunk\_$R$, shrunk\_$Q$, search\_radius)

% \State
% \LineComment{Gets the cells we need to search in this resolution.}
% \State search\_cells $\leftarrow$ expand\_search\_cells(low\_res\_path, search\_radius)


% \State
% \LineComment{Compute DTW over only the cells we need to search.}

% \State dtw $\leftarrow$ array($|$search\_cells$|$)
% \State decision $\leftarrow$ array($|$search\_cells$|$)
% \For{$k, (i, j)$ in enumerate(search\_cells)}
%     \State $k' \leftarrow \argmin\limits_{k''\leftarrow\textrm{try\_find}((p, q), k, \textrm{search\_cells}) \mid (p, q) \in \{(i-1,j), (i,j-1), (i-1,j-1)\}} \textrm{get}(\textrm{dtw}, k'', \infty)$
%     \State $i', j' \leftarrow  \textrm{search\_cells}[k']$
%     \State $\textrm{decision}[k] \leftarrow i', j'$
%     \State $\textrm{dtw}[k] \leftarrow \delta(R[i'], Q[j'])  + \textrm{dtw}[k']$
% \EndFor

% \State
% \LineComment{Compute optimal warping.}
% \State warp\_path\_stack $\leftarrow$ stack()
% \State $k \leftarrow |\textrm{search\_cells}|-1$
% \While{$\textrm{search\_cells}[k] \ne (0, 0)$}
%     \State warp\_path\_stack.insert($(i, j)$)
%     \State $k = \textrm{try\_find}(\textrm{decision}[k], k, \textrm{search\_cells})$
% \EndWhile

% \Return $\textrm{dtw}[-1]$, warp\_path\_stack.pop\_all()
% \EndIf
% \EndProcedure
% \label{alg:fastdtw}
% \end{algorithmic}
% \end{algorithm}





\subsection{Dynamic Time Warping for Navigation}

DTW can be adapted to the context of navigation by using the shortest distance along the graph from node $r_i$ and $q_j$ as the cost function. In continuous scenarios where obstruction is not an issue, the Euclidean distance between the coordinates of any two points in space can be use as a cost function. However in continuous scenarios where obstruction is an issue, one can pre-compute pairwise distances from fixed grid points, and approximate the distance at runtime by finding the closest grid points to $r_i$ and $q_j$. 


One important design consideration is to ensure that the similarity function is invariant to scale, thus making scenarios like indoor \cite{anderson2018vision} and outdoor \cite{Chen19:touchdown,cirik2018following,streetlearn} navigation more comparable. Further, an ideal metric should be invariant to the density of nodes along the trajectories: for instance, in the continuous scenarios, it would be undesirable if the metric changed its value if the sampling rate of the agent changed. To alleviate these issues, we normalize DTW---a sum of at least $|R|$ distance terms--- by a factor of $\frac{1}{|R|\cdot d_{th}}$, where $d_{th}$ is a sampling-rate invariant threshold distance defined for measuring success. Finally, to aid interpretability, we take the negative exponential of its normalized value, resulting in a score bounded between 0 and 1, yielding higher numbers for better performance. In summary, \textit{normalized Dynamic Time Warping} (nDTW) is composed by these operations sequentially applied to DTW, as shown in Eq. \ref{eq:ndtw}.

\begin{equation}
    \textrm{nDTW}(R, Q) = \exp\left(-\dfrac{\textrm{DTW}(R, Q)}{|R|\cdot d_{th}}\right) = \exp\left({-\dfrac{\min\limits_{W \in \mathcal{W}} \sum_{(i_k, j_k) \in W} d(r_{i_k}, q_{j_k})}{|R|\cdot d_{th}}}\right)
    \label{eq:ndtw}
\end{equation}

Since it is directly derived from DTW, nDTW can be exactly computed in quadratic time and space complexity  and approximately computed in linear time and space complexity, as described in the Appendix. In algorithms such as FastDTW where interpolation is required, a simple adaptation---sampling nodes---can be made for discrete environments.

Finally, we notice that, in some tasks, whether or not the trajectory ends close to the goal is key for evaluating performance. This has given rise to multiple ``Success weighted by X" metrics, such as SPL and SED. These metrics harshly penalize---by giving a zero score---any path that does not end within the success threshold $d_{th}$. For such scenarios, we analogously define \textit{Success weighted by normalized Dynamic Time Warping} (SDTW).



\begin{equation}
    \textrm{SDTW}(R, Q) = \textrm{SR}(R, Q) \cdot \textrm{nDTW}(R, Q)
    \label{eq:sdtw}
\end{equation}


\noindent
As we show in the next section using correlation with human judgments, nDTW is superior to path length, edit distance and CLS for quantifying this latter quantity---and thus SDTW should be preferred to SPL, SED and other success weighted measures. Further, there may be different and multiple success criteria for any given task in addition to goal-oriented SR. For example, success could mean picking up an item midway through the path and depositing it near, but not at the end, or selecting a point at the end, as in the spatial description resolution task incorporated into the Touchdown dataset \cite{Chen19:touchdown}. Success is then some soft or hard measure of performance on these actions and SDTW captures well both this success criteria and the fidelity between the agent's movement and the reference path.
